Solving Satisfiability Modulo Counting Exactly with Probabilistic Circuits

Satisfiability Modulo Counting (SMC) is a recently proposed general language to reason about problems integrating statistical and symbolic Artificial Intelligence. An SMC problem is an extended SAT problem in which the truth values of a few Boolean variables are determined by probabilistic inference. Approximate solvers may return solutions that violate constraints. Directly integrating available SAT solvers and probabilistic inference solvers gives exact solutions but results in slow performance because of many back-and-forth invocations of both solvers. We propose KOCO-SMC, an integrated exact SMC solver that efficiently tracks lower and upper bounds in the probabilistic inference process. It enhances computational efficiency by enabling early estimation of probabilistic inference using only partial variable assignments, whereas existing methods require full variable assignments. In the experiment, we compare KOCO-SMC with currently available approximate and exact SMC solvers on large-scale datasets and real-world applications. The proposed KOCO-SMC finds exact solutions with much less time.

==> tex/10.apx.realword.tex <==
\subsection{Dispatching Route Suggestions}


Conventional optimization methods like integer programming or constraint programming prove ineffective in this context as they struggle to represent a suitable objective function for the latent route preference, as noted by~\cite{BRAEKERS2016300}. On the other hand, machine learning models can be employed to learn underlying patterns from historical routes~\cite{junior2021machine}. However, routes generated solely from machine learning models may not adhere to key operational constraints. They might revisit certain locations or fail to visit all locations. Attempts to rectify the output, such as removing redundant locations and randomly adding unvisited locations, through post-processing steps have been made~\cite{DBLP:conf/cpaior/DeudonCLAR18}. Nonetheless, the effectiveness of these post-processing steps is limited.


\subsection{Robust Supply Chain Design}

Existing works in supply chain optimization often gravitate towards mathematical programming approaches. 
However, when delving into more complex scenarios involving stochastic events—such as uncertain demand or supply disruptions—the task becomes considerably more intricate. Specifically, formulating counting constraints, like guaranteeing a certain amount of supplies across multiple vendors under stochastic events, is intractable. 
%
These complexities necessitate innovative approaches that can capture the randomness and dynamism inherent in real-world supply chain systems without sacrificing optimality.

==> tex/5_extend_related.tex <==

\section{Extended Related Works}
Satisfiability Modulo Counting (SMC) was first introduced by \cite{fredrikson2014satisfiability}, aiming to integrate logical satisfiability with probabilistic constraints to address complex decision-making problems. Due to the novelty of this formulation, only a few specialized solvers have been proposed. For instance, \cite{DBLP:proceedings/AAAI24/li-xor-smc} introduced an approximate solver that employs XOR constraints to relax SMC problems, enabling more tractable computations.

Other approaches often focus on specific subclasses of SMC problems. A representative example is Marginal MAP inference, which maximizes a marginal probability over query variables. Its formulation is identical to SMC problems with a single probabilistic constraint. \cite{ChoiAISTATS22} developed exact solvers for Marginal MAP by transforming probabilistic circuits. \cite{marinescu2014and} uses AND-OR search approach to solve the MMAP problem.

The principal idea of our Upper-Lower Bound algorithm is to use the upper and lower bounds of probabilities to avoid unnecessary searches. Similar ideas can be found in branch-and-bound algorithm~\cite{boyd2007branch}, which maintains upper and lower bounds of the objective function to prune suboptimal branches of the search tree, and in alpha-beta pruning~\cite{knuth1975analysis}, which uses bounds on the evaluation of game states to eliminate branches in the game tree that cannot affect the final decision.

==> tex/8_impact.tex <==
\section*{Impact Statement}  
Satisfiability Modulo Counting (SMC) extends traditional Boolean satisfiability by incorporating constraints that involve probability inference (model counting). This extension allows for solving complex problems where both logical and probabilistic constraints must be satisfied. 
SMC has wide applications in supply chain design, shelter allocation, scheduling problems, and many others in Operation Research. For example, in scheduling problems, SMC can ensure that selected schedules meet probabilistic events, while in shelter allocation, it can verify that the accessibility under random disasters is above a specified threshold.


 \noindent\textbf{Limitations} 
 Our Upper-Lower Watch algorithm does not guarantee the tightness of the upper and lower bounds. In the worst case, these bounds may be uninformative, causing \method to degrade to baseline exact solvers. 
 
To address this, we could impose an additional requirement for the probabilistic circuits to be Q-deterministic. In this case, the exact bounds can be inferred, as they become equivalent to Marginal MAP inference. We can then leverage \cite{ChoiAISTATS22} to reduce the computation to a probabilistic circuit traversal.
%
However, due to the limitations of knowledge compilers, compiling a complex distribution may: require excessive time or space and be incompatible with the structural requirements, as many knowledge compilers do not support them.
